Nonlinear enthalpy transformation for transient convective phase change in Smoothed Particle Hydrodynamics (SPH)

A three-dimensional model is presented for the prediction of solidification behavior using a nonlinear transformation of the enthalpy equation in a Smoothed Particle Hydrodynamics (SPH) discretization. The effect of phase change in the form of release and absorption of latent heat is implemented implicitly as variable source terms in the enthalpy calculation. The developed model is validated against various experimental, analytical, and numerical results from the literature. Results confirm accuracy and robustness of the new procedure. Finally, the SPH model is applied to a study of suspension plasma spraying (SPS) by predicting the impact and solidification behavior of molten ceramic droplets on a substrate.

==> matlab.tex <==
Using the information gathered from these simulations, a simplified Matlab model was developed to to simulate coating fromation based on the SPS data of \cite{Farrokhpanah_16_2} which includes one million droplet impacts sprayed over $0.61 s$. The simplified model assumes that solidified splats are in the form of discs on the substrate. The tangential component of impact velocities is neglected. Results of simulations of the previous sections suggest that when a droplet at high temperature impacts an uneven surface, there is a high chance for void formation, of a size similar to the height of the void. This has been included here, by making the assumption that droplets impacting the surface at high temperature will contribute to the formation of small voids.

Application of the simplified model to the case of the five droplets of table \ref{tab:SPS_IMP_1} is shown in figure \ref{fig:SPS_IMP_23}. It can be seen that the overall behavior of the impacts is predicted reasonably well, as the high and low points in both simulation and prediction are close. The code was then applied to the one million droplets from the SPS dataset. Substrate coating at multiple scales is shown in Figure \ref{fig:SPS_IMP_24}.

